Unveiling Secrets of Brain Function With Generative Modeling: Motion Perception in Primates & Cortical Network Organization in Mice

This Dissertation is comprised of two main projects, addressing questions in neuroscience through applications of generative modeling. Project #1 (Chapter 4) explores how neurons encode features of the external world. I combine Helmholtz's "Perception as Unconscious Inference" -- paralleled by modern generative models like variational autoencoders (VAE) -- with the hierarchical structure of the visual cortex. This combination leads to the development of a hierarchical VAE model, which I test for its ability to mimic neurons from the primate visual cortex in response to motion stimuli. Results show that the hierarchical VAE perceives motion similar to the primate brain. Additionally, the model identifies causal factors of retinal motion inputs, such as object- and self-motion, in a completely unsupervised manner. Collectively, these results suggest that hierarchical inference underlines the brain's understanding of the world, and hierarchical VAEs can effectively model this understanding. Project #2 (Chapter 5) investigates the spatiotemporal structure of spontaneous brain activity and its reflection of brain states like rest. Using simultaneous fMRI and wide-field Ca2+ imaging data, this project demonstrates that the mouse cortex can be decomposed into overlapping communities, with around half of the cortical regions belonging to multiple communities. Comparisons reveal similarities and differences between networks inferred from fMRI and Ca2+ signals. The introduction (Chapter 1) is divided similarly to this abstract: sections 1.1 to 1.8 provide background information about Project #1, and sections 1.9 to 1.13 are related to Project #2. Chapter 2 includes historical background, Chapter 3 provides the necessary mathematical background, and finally, Chapter 6 contains concluding remarks and future directions.

==> Bibliography.tex <==
\begin{thebibliography}{99}
\setlength{\parskip}{1em}

\bibitem{Agrawal1} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 1.
\bibitem{Bloembergen} N. Bloembergen, {\em Nonlinear Optics} (Benjamin,
Reading, MA, 1977).
\bibitem{Shen} Y.R. Shen, {\em Principles of Nonlinear Optics} (Wiley, New
York, 1984).
\bibitem{Butcher} P.N. Butcher and D.N. Cotter, {\em The Elements of
Nonlinear Optics} (Cambridge University Press, Cambridge, UK, 1990).
\bibitem{Boyd} R.W. Boyd, {\em Nonlinear Optics} (Academic Press, San Diego,
CA, 1992).
\bibitem{Newell} A.C. Newell and J.V. Moloney {\em Nonlinear Optics (Advanced Topics in the Interdisciplinary Mathematical Sciences)} (Westview Press, Boulder, CO, April 1992). 
\bibitem{Marcuse} D. Marcuse,{\em Light Transmission Optics} (Van Nostrand
Reinhold, New York, 1982), Chaps. 8 and 12.
\bibitem{Agrawal2} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 2.
\bibitem{Diament} P. Diament, {\em Wave Transmission and Fiber Optics}
(Macmillan, New York, 1990).
\bibitem{Zakharov} V.E. Zakharov and A.Shabat, Sov. Phys. JETP 
\textbf{34}, 62 (1972)
\bibitem{Hardin} R.H. Hardin and F.D. Tappert, SIAM
Rev. Chronicle \textbf{15}, 423 (1973).
\bibitem{Fisher} R.A.Fisher and
W.K. Bischel, Appl. Phys. Lett. \textbf{23}, 661 (1973); J. Appl. Phys
\textbf{46}, 4921 (1975).
\bibitem{Cooley} J.W. Cooley and J.W. Tukey,
Math. Comput. \textbf{19}, 297 (1965).
\bibitem{Trebino} R. Trebino, D.J. Kane, "Using phase retrieval to measure
the intensity and phase of ultrashort pulses: frequency resolved optical gating," J. Opt. Soc. Am. B \textbf{10}, 1101 (1993). 
\bibitem{Kanejqe} D.J. Kane, R. Trebino, "Characterization of Arbitrary Femtosecond Pulses Using Frequency-Resolved Optical Gating," IEEE J. Quant. Elect. \textbf{29}, 571 (1993). 
\bibitem{Kaneoptlett} D.J. Kane, R. Trebino, "Single-shot measurement of the intensity and phase of an arbitrary ultrashort pulse  by using frequency-resolved optical gating," Opt. Lett. \textbf{10}, 1101 (1993).
\bibitem{OShealett}P. O'Shea, M. Kimmel, X. Gu, R. Trebino, "Highly simplified device for ultrashort-pulse measurement," Opt. Lett. \textbf{26}, 932 (2001).
\bibitem{Agrawal3} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 3.
\bibitem{Agrawal4} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 4.
\bibitem{Agrawal10} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 10.
\bibitem{Agrawal7} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 7.
\bibitem{Agrawal6} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 6.
\bibitem{Stolen} R.H. Stolen, E.P. Ippen, and A.R. Tynes,
Appl. Phys. Lett. \textbf{20}, 62 (1972). 
\bibitem{Ippen} E.P. Ippen and R.H. Stolen, Appl. Phys. Lett. \textbf{21}, 
539 (1972). 
\bibitem{Smith} R.G. Smith, Appl. Opt. \textbf{11}, 2489 (1972).
\bibitem{Agrawal9} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 9.
\bibitem{Agrawal8} G.P. Agrawal, {\em Nonlinear Fiber Optics} (Academic
Press, San Diego, CA, 2001), Chap. 8.
\bibitem{hart1} D.L. Hart, Arthur F. Judy, Rajarshi Roy and James W. Beletic, Phys. Rev. E \textbf{57}, 4757 (1998); D.L. Hart, Arthur F. Judy, T.A.B. Kennedy, Rajarshi Roy and K. Stoev, Phys. Rev. A \textbf{50}, 1807 (1994).   
\bibitem{ito} K. Ito, {\em Lectures on Stochastic Processes} (Tata Institute of Fundamental Research, Bombay, 1960).
\bibitem{stratanovich} R.L. Stratanovich, {\em Topics in the Theory of Random Noise}, Vols I. and II. (Gordon \& Breach, New York, 1963).
\bibitem{risken} H. Risken, {\em The Fokker-Planck Equation} (Springer-Verlag, Berlin, 1989).
\bibitem{werner2} M.J. Werner and P.D. Drummond, J. Comput. Phys. \textbf{132}, 312 (1997).
\bibitem{drummond1} P.D. Drummond and I.K. Mortimer, J. Comput. Phys. \textbf{93}, 144 (1991).
\bibitem{carter3} S.J. Carter, Phys. Rev. A. \textbf{51}, 3274 (1995).
\bibitem{thompson1} J.R. Thompson and Rajarshi Roy, Phys. Rev. A \textbf{43}, 4987 (1991).
\bibitem{boxmuller} W.H. Press, S.A. Teukolsky, W.T. Vetterling and B.P. Flannery, {\em Numerical Recipes in Fortran: The Art of Scientific Computing} (Cambridge University Press, Cambridge, 1992).
\bibitem{headley} C. Headley, G.P. Agrawal, IEEE J. Quantum Electron. \textbf{QE-31}, 2058 (1995), C. Headley, G.P. Agrawal J. Opt. Soc. Am. B. \textbf{13}, 2170 (1995).
\bibitem{perlmutter1} S.H. Perlmutter, M.D. Levenson, R.M. Shelby and
M.B. Weisman, Phys. Rev. Lett. \textbf{61} 1388, 1988.
\bibitem{abdullaev} F. Kh. Abdullaev, J.H. Hensen, S. Bischoff and M.P. Sorensen, J. Opt. Soc. Am. B. \textbf{15}, 2424 (1998); F. Kh. Abdullaev, J.G. Caputo, and Nikos Flytzanis, Phys. Rev E. \textbf{50}, 1552 (1994).
\bibitem{glenn} William H. Glenn, IEEE J. Quantum Electron. \textbf{QE-25}, 1218 (1989).
\bibitem{Trebinobook} R. Trebino. {\em Frequency-Resolved Optical Gating: The Measurement of Ultrashort Laser Pulses} (Kluwer Academic 2002).
\bibitem{Agrawal} G.P. Agrawal {\em Nonlinear Fiber Optics} (Academic,
San Diego, 2001).
\bibitem{Dudley} J.M. Dudley, X. Gu, L. Xu, M. Kimmel, E. Zeek, P. O'Shea, R. Trebino, S. Coen, R.S. Windeler, "Cross-correlation frequency resolved optical gating analysis of broadband continuum generation in photonic crystal fiber: simulations and experiments," Opt. Express \textbf{10}, 1215 (2002).
\bibitem{Liu1} Q.D. Liu, J.T. Chen, Q.Z. Wang, P.P. Ho, and R.R. Alfano, "Single pulse degenerate-cross-phase modulation in a single-mode optical fiber," Opt. Lett. \textbf{20}, 542 (1995).
\bibitem{Sylvestre} T. Sylvestre, H. Maillotte, E. Lantz, and D. Gindre "Combined spectral effects of pulse walk-off and degenerate cross-phase modulation in birefringent fibers", Journal of Nonlinear Optical Physics and Materials 6, 313-320 (1997).
\bibitem{Liu2} Q.D. Liu, L. Shi, P.P. Ho, R.R. Alfano, R.J. Essiambre, and G.P. Agrawal, "Degenerate cross-phase modulation of femtosecond laser pulses in a birefringent single-mode fiber," IEEE Photon. Tech. Lett. \textbf{9}, 1107 (1997). 
\bibitem{Omenetto1} F.G. Omenetto, B.P. Luce, D. Yarotski and A.J. Taylor, "Observation of chirped soliton dynamics at l= 1.55 mm in a single-mode optical fiber with frequency-resolved optical gating," Opt. Lett. \textbf{24}, 1392 (1999).
% 1.55 micron regime - check for more recent papers by Omenetto use both web-sci and inspec
\bibitem{Omenetto2} F.G. Omenetto, Y. Chung, D. Yarotski, T. Shaefer, I. Gabitov and A.J. Taylor, "Phase analysis of nonlinear femtosecond pulse propagation and self-frequency shift in optical fibers," Opt. Commun. \textbf{208}, 191 (2002). 
\bibitem{Omenetto3} F.G. Omenetto, J.W. Nicholson, B.P. Luce, D. Yarotski, A.J. Taylor, "Shaping, propagation and characterization of ultrafast pulses in optical fibers," Appl. Phys. B \textbf{70}[Suppl.], S143 (2000).
\bibitem{Nishizawa1} N. Nishizawa and T. Goto, "Experimental analysis of ultrashort pulse propagation in optical fibers around zero-dispersion region using cross-correlation frequency resolved optical gating," Opt. Express \textbf{8}, 328 (2001).
\bibitem{Nishizawa2} N. Nishizawa and T. Goto, "Trapped pulse generation by femtosecond soliton pulse in birefringent optical fibers," Opt. Express \textbf{10}, 256 (2002).
\bibitem{Nishizawa3} N. Nishizawa and T. Goto, "Characteristics of pulse trapping by use of ultrashort soliton pulses in optical fibers across the zero-dispersion wavelength," Opt. Express \textbf{10}, 1151 (2002).
\bibitem{Nishizawa4} N. Nishizawa and T. Goto, "Ultrafast all optical switching by use of pulse trapping across zero-dispersion wavelength," Opt. Express \textbf{11}, 359 (2003).
% All of Nishizawa and Goto papers are related to 1.3 micron experiments and simulations.
\bibitem{Ogawa}, K. Ogawa, M.D. Pelusi, "Characterization of ultrashort optical pulses in a dispersion-managed fiber link using two-photon absorption frequency-resolved optical gating," Opt. Commun. \textbf{198}, 83-87 (2001).
\bibitem{Altes} R.A. Altes, "Detection, estimation, and classification
with spectrograms," J. Acoust. Soc. Am. \textbf{67}(4), 1232 (1980).
\bibitem{Christian} A. Christian Silva, "GRENOUILLE - Practical Issues," unpublished.
\bibitem{Mejia} J. Garduno-Mejia, A.H. Greenaway, and D.T. Reid, "Designer
femtosecond pulses using adaptive optics," Opt. Express \textbf{11}
2030 (2003).
\bibitem{OSheaexpress1} P. O'Shea, M. Kimmel, X. Gu, R. Trebino, "Increased-bandwidth in ultrashort-pulse measurement using an angle-dithered nonlinear-optical crystal," Opt. Express \textbf{7}, 342 (2000).
\bibitem{OSheaexpress2} P. O'Shea, M. Kimmel, R. Trebino, "Increased phase-matching bandwidth in simple ultrashort-laser-pulse measurements," J. Opt. B \textbf{4}, 44 (2002).
\bibitem{Akturk} S. Akturk, M. Kimmel, P. O'Shea, R. Trebino, "Measuring pulse-front tilt in ultrashort pulses using GRENOUILLE", Opt. Express \textbf{11}, 491 (2003).
\bibitem{Blow} K. J. Blow, D. Wood, "Theoretical Description of Transient Stimulated Raman Scattering in Optical Fibers," IEEE J. Quant. Elect. \textbf{25}, 2665 (1989).
\bibitem{Stolen2} R.H. Stolen, J.P. Gordon, W.J. Tomlinson,
J. Opt. Soc. Am. B \textbf{6}, 1159 (1989).
\bibitem{Mamyshev} P.V. Mamyshev and S.V. Chernikov, Sov. Lightwave
Commun. \textbf{2}, 97 (1992).
\bibitem{Headleythesis} C. Headley III, \em{Ultrafast Stimulated Raman
Scattering in Optical Fibers}, Ph.D. Thesis, University of Rochester,
NY (1995).
\end{thebibliography}


==> Dedication.tex <==
%Dedication

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{.5in}

\begin{center}
\large{Dedication}
\end{center} 

If needed.


==> Foreword.tex <==
%Foreword

\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }
 
\vspace{.5in}

\begin{center}
\large{Foreword} 
\end{center} 

If needed.

